Federated Natural Policy Gradient and Actor Critic Methods for Multi-task Reinforcement Learning

Federated reinforcement learning (RL) enables collaborative decision making of multiple distributed agents without sharing local data trajectories. In this work, we consider a multi-task setting, in which each agent has its own private reward function corresponding to different tasks, while sharing the same transition kernel of the environment. Focusing on infinite-horizon Markov decision processes, the goal is to learn a globally optimal policy that maximizes the sum of the discounted total rewards of all the agents in a decentralized manner, where each agent only communicates with its neighbors over some prescribed graph topology. We develop federated vanilla and entropy-regularized natural policy gradient (NPG) methods in the tabular setting under softmax parameterization, where gradient tracking is applied to estimate the global Q-function to mitigate the impact of imperfect information sharing. We establish non-asymptotic global convergence guarantees under exact policy evaluation, where the rates are nearly independent of the size of the state-action space and illuminate the impacts of network size and connectivity. To the best of our knowledge, this is the first time that near dimension-free global convergence is established for federated multi-task RL using policy optimization. We further go beyond the tabular setting by proposing a federated natural actor critic (NAC) method for multi-task RL with function approximation, and establish its finite-time sample complexity taking the errors of function approximation into account.

==> DNPG.tex <==
\section{inexact entropy-regularized FedNPG/FedNPG}\label{sec_app:DNPG+inexact}

In this paper, we also consider the inexact case where exact Q-function $\mQ_\tau^{(t)}$ (resp. $\mQ^{(t)}$) are unavailable in each step of entropy-regularized FedNPG (resp. FedNPG), and we could only compute their approximation $\vq_\tau^{(t)}$ (resp. $\vq^{(t)}$).
To avoid redundancy we put the inexact version of both entropy-regularized FedNPG and DNPG into Alg.~\ref{alg:DNPG_inexact}, where we define
\begin{equation}\label{q_tau}
    \vq_\tau^{(t)}\triangleq \left( q_{\tau,1}^{\pi_1^{(t)}},\cdots, q_{\tau,N}^{\pi_N^{(t)}}\right)^\top\,,
\end{equation}
where $q_{\tau,1}^{\pi_n^{(t)}}$ is an approximation of $Q_{\tau,1}^{\pi_n^{(t)}}$ ($n\in[N]$). 

\begin{algorithm}[H]
    \caption{entropy-regularized FedNPG (FedNPG when $\tau=0$) with inexact policy evaluation}
    \label{alg:DNPG_inexact}
    \begin{algorithmic}[1] 
        \STATE \textbf{Input:}  learning rate $\eta\geq 0$, iteration number $T\in\NN_+$, mixing matrix $\mW\in\R^{N\times N}$, regularization coefficient $\tau>0$.

        \STATE \textbf{Initialize:} $\vpi^{(0)}$, $\mT^{(0)}=\vq_\tau^{(0)}\approx\mQ_\tau^{(0)}$.
        
        \FOR{$t=0, 1, \cdots T-1$} %%%%%%
            \STATE Compute $\vq_\tau^{(t+1)}\approx\mQ_\tau^{(t+1)}$.

            \STATE Update the policy for each $(s,a)\in \mathcal{S}\times \mathcal{A}$:
            \begin{equation}\label{eq:update_marl_inexact}
                \log\vpi^{(t+1)}(a|s)=\left(1-\frac{\eta \tau}{1-\gamma}\right)\mW\log\vpi^{(t)}(a|s)+\frac{\eta}{1-\gamma}\mT^{(t)}(s,a)- \log\vz^{(t)}(s)\,,
            \end{equation}
            where $\vz^{(t)}(s)=\sum_{a'\in\mathcal{A}}\exp\left\{\left(1-\frac{\eta \tau}{1-\gamma}\right)\mW\log\vpi^{(t)}(a'|s)+\frac{\eta}{1-\gamma}\mT^{(t)}(s,a')\right\}$.

            \STATE Update the global Q-function estimate for each $(s,a)\in \mathcal{S}\times \mathcal{A}$:
            \begin{equation}\label{eq:Q_tracking_inexact}
                \mT^{(t+1)}(s,a)=\mW\left(\mT^{(t)}(s,a)+\vq_\tau^{(t+1)}(s,a)-\vq_\tau^{(t)}(s,a)\right)\,.
            \end{equation}
        \ENDFOR 
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}

%Recall that $\mQ_\tau^{(t)}\triangleq \left( Q_{\tau,1}^{\pi_1^{(t)}},\cdots, Q_{\tau,N}^{\pi_1^{(t)}}\right)^\top$.
We define
$e_n\in\R$ as
\begin{equation}\label{eq:delta_n}
    e_n\triangleq \norm{Q_{\tau,n}^{\pi_n^{(t)}}-q_{\tau,n}^{\pi_n^{(t)}}}_\infty\,,\quad n\in[N]\,,
\end{equation}
and we let $\ve=(e_1,\cdots,e_n)^\top$.


==> alg.tex <==
%\section{Omitted Algorithms}\label{sec_app:alg}

\section{Development of~\alg}\label{sec_app:FedNAC}

% For any policy $\pi$, we let $d^\pi_{s_0}$ denote the discounted state visitation distribution of $\pi$ given an initial state $s_0 \in \mathcal{S}$, i.e.,
% \begin{equation}\label{eq:d_s0} %\tag{$d_{s_0}$}
%     \forall s\in\mathcal{S}: \quad d^\pi_{s_0}(s)\coloneqq (1-\gamma)\sum_{t=0}^\infty \gamma^t\mathbb{P}(s_t=s|s_0)\,.
% \end{equation}


% For a distribution $\rho\in\Delta(\S)$, we define $d_\rho^\pi(s)=\E_{s_0\sim\rho}[d_{s_0}^\pi(s)]$. We also define the \textit{state-action visitation distribution} $\bar{d}^\pi_\rho$ as 
% % $$\bar{d}^\pi_{\rho}(s,a)\coloneqq d^\pi_{\rho}(s)\pi(a|s) =(1-\gamma)\E_{s_0\sim\rho}\left[\sum_{t=0}^\infty \gamma^t\mathbb{P}(s_t=s, a_t=a|s_0)\right].$$
% \begin{align}\label{eq:sa_vis}
%     \bar{d}^\pi_{\rho}(s,a)\coloneqq& d^\pi_{\rho}(s)\pi(a|s)
%     =(1-\gamma)\E_{s_0\sim\rho}\left[\sum_{t=0}^\infty \gamma^t\mathbb{P}(s_t=s, a_t=a|s_0)\right]\,.
% \end{align}

% Furthermore, we extend the definition of $\bar{d}^\pi_\rho$ by specifying the initial state-action distribution $\nu\in\Delta(\S\times\A)$ and define % $\tilde{d}^\pi_{\nu}(s,a)\coloneqq (1-\gamma)\underset{(s_0,a_0)\sim\nu}{\E}\left[\sum_{t=0}^\infty \gamma^t\mathbb{P}(s_t=s, a_t=a|s_0,a_0)\right].$
% \begin{equation}\label{eq:sa_vis_extend}
%     %\forall (s,a)\in\S\times \A:\quad  
%     \tilde{d}^\pi_{\nu}(s,a)\coloneqq (1-\gamma)\underset{(s_0,a_0)\sim\nu}{\E}\left[\sum_{t=0}^\infty \gamma^t\mathbb{P}(s_t=s, a_t=a|s_0,a_0)\right]\,.
% \end{equation}

Our proposed federated NAC method {\alg} could be seen as a decentralized version of Q-NPG method~\citep{agarwal2021theory,yuan2022linear}, which we briefly review as follows.

\paragraph{Q-NPG method.} Q-NPG is a sample version of NPG with function approximation which is suitable for the case where $\S$ or $\A$ is large or infinite. 
We consider the policy with function approximation under softmax parameterization \eqref{eq:param_fa}.
% , which takes the following form:
% \begin{equation}\label{eq:param_fa}
%     %\forall (s,a)\in\S\times\A, \forall\vxi\in\R^p:\quad 
%     f_\xi(a|s)=\frac{\exp(\phi^\top(s,a)\vxi)}{\sum_{a'\in\A}\exp(\phi^\top(s,a')\vxi)},
% \end{equation}
% for all $(s,a)\in\S\times\A$ and $\vxi\in\R^p$, where
% $\phi: \S\times\A\rightarrow \R^p$ is a known feature mapping, and $\varPhi$ is the corresponding feature matrix. We assume $\phi$ is bounded over $\S\times\A$, i.e., there exists $C_\phi>0$ such that $\norm{\phi(s,a)}_2\leq C_\phi$ holds for all $(s,a)\in\S\times\A$. 
% Given any $\vw\in\R^p$, $Q:\S\times\A\rightarrow \R$ and a probability distribution $\zeta\in\Delta(\S\times\A)$, we define the \textit{function approximation error} $\ell(\vw,Q,\zeta)$ as follows:
% \begin{equation}\label{eq:l}
%     \ell(\vw,Q,\zeta)\coloneqq \E_{(s,a)\sim \zeta}\left[\left(\vw^\top\phi(s,a)-Q(s,a)\right)^2\right].
% \end{equation}

Given an approximate solution $\vw^{(t)}$ for minimizing the function approximation error $\ell(\vw,Q^{f_{\xi^{(t)}}},\tilde d_\nu^{f_{\xi^{(t)}}})$ (see \eqref{eq:l}), the Q-NPG update rule $\vxi^{(t+1)}=\vxi^{(t)}+\alpha \vw^{(t)}$, when plugged in parameterization~\eqref{eq:param_fa}, results in the following policy update rule when we set $\alpha=\eta/(1-\gamma)$:
\begin{equation}\label{eq:Q_NPG_policy_update}
    f^{(t+1)}(a|s)\propto f^{(t)}(a|s)\exp\left(\frac{\eta\phi^\top(s,a)\vw^{(t)}}{1-\gamma}\right)\,,
\end{equation}
which could be seen as the function approximation version of the update rule~\eqref{eq:update_npg_vanilla} of vanilla NPG method.


\paragraph{Federated NAC method.} \textit{\alg} (describe in Section~\ref{sec:nac_ext})~is presented in Algorithm~\ref{alg:actor_critic}, whose subroutines are written in Algorithm~\ref{alg:critic},~\ref{alg:sampler}. \ In each iteration $t$ of~\alg, each agent $n$ updates the critic parameter $\vw_n^{(t)}$ locally using Algorithm~\ref{alg:critic}, which aims to minimize $\ell(\vw,Q_n^{(t)},\tilde d_n^{(t)})$ by stochastic gradient descent. Note that since we don't know the Q-function $Q_n^{(t)}$ in the gradients, we need to invoke Algorithm~\ref{alg:sampler}~\citep[Algorithm~3]{yuan2022linear} to give an unbiased estimate $\widehat Q_n^{(t)}(s,a)$, where $(s,a)$ is sampled from $\tilde d_n^{(t)}$ (cf.~Theorem~\ref{thm:sampler}). As a consequence, in line~4 of Algorithm~\ref{alg:critic}, we have 
\begin{equation}\label{eq:unbias_gd}
    \E \left[\widehat{\nabla}_w \ell(\widetilde{\vw}_k,\widehat{Q}^\pi,\tilde{d}^{f_\xi})\right]=\nabla_w \ell(\widetilde{\vw}_k,\widehat{Q}^\pi,\tilde{d}^{f_\xi})\,.
\end{equation}
In each actor iteration, agents share with their neighbors actor and critic parameters, where the tracking scheme is also used.


%, and $\varPhi$ is the corresponding feature matrix 
\begin{algorithm}[ht]
    \caption{Federated Natural Actor-Critic (\alg)}
    \label{alg:actor_critic}
    \begin{algorithmic}[1] 
        \STATE \textbf{Input:}  % actor parameter $\xi_0$, % critic parameter $\vxi_0$, 
        number of actor iterations $T$, number of critic iterations $K$,
        actor learning rate $\alpha$, %$\{\alpha_t\}_{t=0}^{T-1}$, 
        critic learning rate $\beta$, discounted factor $\gamma\in [0,1)$
        \STATE \textbf{Initialization:} initial state-action distribution $\nu$, actor parameter $\vxi^{(0)}=(\vxi^{(0)\top}_{1},\cdots,\vxi^{(0)\top}_{N})^\top\in\R^{N\times p}$, $\vh^{(-1)}=\vw^{(-1)}=\vzero\in\R^{N\times p}$
        
        \FOR{$t=0, \cdots, T-1$} %%%%%%
            \STATE Critic update: $\vw^{(t)}_n=$ \, \critic ($K$, $\nu$, $\vxi^{(t)}_n$, $\gamma$, $\beta$, $r_n$), $n\in[N]$ (Algorithm \ref{alg:critic})
            
            \STATE Update the critic parameter for estimating the global Q-function:
            \begin{equation}\label{eq:GT}
                \vh^{(t)}=\mW\left(\vh^{(t-1)}+\vw^{(t)}-\vw^{(t-1)}\right)
            \end{equation}
            
            \STATE Actor update:
            \begin{equation}\label{eq:actor_update}
                \vxi^{(t+1)}=\mW\left(\vxi^{(t)}+\alpha \vh^{(t)}\right)
            \end{equation}
        \ENDFOR 
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}


\begin{algorithm}[ht]
    \caption{\critic $(K, \nu, \vxi, \gamma, \beta, r)$: sample-based regression solver to minimize $\ell(\vw,Q_n^{(t)},\tilde d_n^{(t)})$ }
    \label{alg:critic}
    \begin{algorithmic}[1] 
        \STATE \textbf{Initialize:} critic parameter $w_0\in\R^p$
        \FOR{$k=0,\cdots, K-1$}
            \STATE Sampling: $(s_k, a_k), \widehat{Q}^\pi(s_k,a_k)=$\sampler($\nu, f_\xi, \gamma$, $r$) (Algorithm~\ref{alg:sampler}) 
            \STATE Compute the stochastic gradient estimator of $L_Q$: 
            \begin{equation}\label{eq:sg_LQ}
                \widehat{\nabla}_w \ell(\widetilde{\vw}_k,\widehat{Q}^\pi,\tilde{d}^{f_\xi})=2\left(\widetilde{\vw}_k^\top \phi(s_k,a_k)-\widehat{Q}^\pi(s_k,a_k)\right)\phi(s_k,a_k)
            \end{equation}
            \STATE Critic Update: $\widetilde{\vw}_{k+1}=\widetilde{\vw}_k-\beta \widehat{\nabla}_w \ell(\widetilde{\vw}_k,\widehat{Q}^\pi,\tilde{d}^{f_\xi})$
        \ENDFOR
        \STATE \textbf{Output:} $\vw_{\text{out}}=\frac{1}{K}\sum_{k=1}^K \widetilde{\vw}_k$
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}

\begin{algorithm}[ht]
    \caption{\sampler $(\nu, \pi, \gamma, r)$}
    \label{alg:sampler}
    \begin{algorithmic}[1] 
        \STATE \textbf{Initialize:} $(s_0,a_0)\sim \nu$, time step $h,t=0$, variable $X\sim$ Bernoulli($\gamma$)
        \WHILE{$X=1$}
            \STATE Sample $s_{h+1}\sim P(\cdot|s_h,a_h)$
            \STATE Sample $a_{h+1}\sim \pi(\cdot|s_{h+1})$
            \STATE $h\leftarrow h+1$
            \STATE $X\sim$ Bernoulli($\gamma$)
        \ENDWHILE
        \STATE Set $\widehat{Q}^\pi(s_h,a_h)=r(s_h,a_h)$, $X\sim$ Bernoulli($\gamma$), $t=h$
        \WHILE{$X=1$}
            \STATE Sample $s_{t+1}\sim P(\cdot|s_t,a_t)$
            \STATE Sample $a_{t+1}\sim \pi(\cdot|s_{t+1})$
            \STATE $\widehat{Q}^\pi(s_h,a_h)\leftarrow \widehat{Q}^\pi(s_h,a_h)+r(s_{t+1},a_{t+1})$
            \STATE $t\leftarrow t+1$
            \STATE $X\sim$ Bernoulli($\gamma$)
        \ENDWHILE
        \STATE \textbf{Output:} $(s_h,a_h)$ and $\widehat{Q}^\pi(s_h,a_h)$
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}

==> experiments.tex <==

\newpage
\section{Numerical experiments}\label{sec_app:exp}
\subsection{Setup and Results}

\paragraph{Experimental setup.} We study the empirical performance of FedNPG (Algorithm~\ref{alg:DNPG_exact}) and entropy-regularized FedNPG (Algorithm~\ref{alg:EDNPG_exact}) on a $K\times K$ GridWorld problem. To be specific, the collective goal of $N$ agents is to learn a global optimal policy to follow a predetermined path which starts at the top left corner and ends at the bottom right corner. However, each agent only has access to partial information about the whole map: in figure~\ref{fig:gridworld} (where we take $N=3$ and $K=9$ as an example), agent $n$ explores on map $n$, $n\in[N]$. After taking an action, only when the agent is at the shaded positions can it get reward 1, otherwise it gets 0. We stipulate the action space of all agents to be $\A=\{\text{right},\text{down}\}$, i.e. movement is allowed only to the right or down. If an agent takes an action that will lead it out of the boarder of the map, we stipulate the agent's state doesn't change and receive reward 0.  Each agent starts at the top left corner. 
To learn a shared policy to follow the path, we aim to maximize the average value function of all agents.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=.75\linewidth]{figures/gridworld.jpeg}
\caption{Gridworld experiement. $N$ agents ($N=3$ here) aim to learn a shared policy to follow a predetermined path, which is the red dashed line in the complete map. Each agent only has access to partial information about the path and gets reward 1 only at the shaded positions and 0 at other positions. Each agent starts at the top left corner.
}\label{fig:gridworld}
\end{figure}

\paragraph{Results.} In the following we discuss the empirical results of our algorithms. In all the experiments, we fix the discounted factor $\gamma=0.99$. In our experiments, we also don't require the mixing matrix to strictly adhere to Assumption~\ref{asmp:mixing matrix}. In Figure~\ref{fig:change_K}, we validate the effectiveness of vanilla FedNPG and entropy-regularized FedNPG across different map size $K$, where we set $\tau=0,0.005,0.05$, $\eta=0.1$, $N=10$, and use a \textit{standard ring graph} where agent $n$ receives information from agent $n+1$ for $n\in[N-1]$, and agent $N$ receives information from agent 1, and we set all the weights on each edge of the communication graph to be 0.5. The corresponding mixing matrix of the standard ring graph is as follows:
\begin{equation}\label{eq:standard_ring}
    \mW=\begin{pmatrix}
        0.5 & 0.5 & 0 & 0 & \cdots & 0 & 0 \\
        0 & 0.5 & 0.5 & 0 & \cdots & 0 & 0 \\
        0 & 0 & 0.5 & 0.5 & \cdots & 0 & 0 \\
        \vdots & \vdots & \vdots & \vdots & & \vdots & \vdots \\
        0 & 0 & 0 & 0 & \cdots & 0.5 & 0.5 \\
        0.5 & 0 & 0 & 0 & \cdots & 0 & 0.5
    \end{pmatrix}\,.
\end{equation}
Here, $\mW$ in \eqref{eq:standard_ring} satisfies the double stochasticity assumption but is not symmetric. 

\begin{figure}[!htb]
\vspace*{-.5em}
  \centering
  \subfigure[$\tau=0$]{\label{subfig:change_K_tau=0}
  \includegraphics[width=.4\linewidth]{figures/change_K_tau=0.pdf}} 
  \subfigure[$\tau=0.005$]{\label{subfig:change_K_tau=0.005}
  \includegraphics[width=.4\linewidth]{figures/change_K_tau=0.005.pdf}} 
  %\vspace*{-.6em}
  \caption{ \textbf{Changing map size $K$.} we let $\tau=0,0.005$ and change $K$ for each $\tau$. We plot the curves of $(V^\star_\tau-\overline{V}^{(t)}_\tau)/V^\star_\tau$ changing with the iteration number. We can see that both vanilla and entropy-regularized NPG converges to the optimal value function in a few iterations, and the convergence speed is almost the same across different $K$.
  }\label{fig:change_K}
\end{figure}

Figure~\ref{fig:change_K} illustrates the normalized sub-optimality gap $(V^\star_\tau-\overline{V}^{(t)}_\tau)/V^\star_\tau$ with respect to the iteration number. It can be seen that both vanilla and entropy-regularized NPG converge to the optimal value function in a few iterations, and the convergence speed is almost the same across different $K$, i.e. the impact of $K$ on the convergence speed is minimal.

\begin{figure}[!htb]
\vspace*{-.5em}
  \centering
  \subfigure[$K=10$]{\label{subfig:change_N_K=10}
  \includegraphics[width=.32\linewidth]{figures/change_N_K=10.pdf}}  
  \subfigure[$K=20$]{\label{subfig:change_N_K=20}
  \includegraphics[width=.32\linewidth]{figures/change_N_K=20.pdf}} 
  \subfigure[$K=30$]{\label{subfig:change_N_K=30}
  \includegraphics[width=.32\linewidth]{figures/change_N_K=30.pdf}} 
  %\vspace*{-.6em}
  \caption{ \textbf{Changing number of agents $N$.} we let $K=10,20,30$ and change $N$ for each $K$. We plot the curves of value functions changing with the iteration number. The green dashed line represents the optimal value. We can see that the convergence speed decreases as $N$ increases. Same as before, the convergence speed is insensitive to the change of $K$.
  }\label{fig:change_N}
\end{figure}

In Figure~\ref{fig:change_N}, we study the performance of our algorithms when the number of agents $N$ varies. We set $K=10,20,30$, $\tau=0.005$, $\eta=0.1$ and the communication graph to be the standard ring graph. We can see that the convergence speed decreases as $N$ increases. Same as before, the convergence speed is insensitive to the change of $K$.

In Figure~\ref{fig:change_top}, we illustrate the effect of the communication network topology to our algorithms. To be specific, we change the number of neighbors of each agent (i.e., the number of non-zero entries in each row of $\mW$) and (i) randomly generalize the weights of the graph such that each row of $\mW$ sum up to 1, i.e.,$\mW\vone=\vone$, see Figure~\ref{subfig:change_top_random}; (ii) set the non-zero entries in each row of $\mW$ all to be $\frac{1}{\text{number of neighbors}}$, see Figure~\ref{subfig:change_top}. We fix $\eta=0.1$, $K=10$, $\tau=0.005$. We plot the curves of value functions changing with the iteration number. The green dashed line represents the optimal value. For both \ref{subfig:change_top_random} and \ref{subfig:change_top}, the convergence speed increase as number of neighbors of each agent increases. FedNPG performs better when using equal weights.
\begin{figure}[!htb]
\vspace*{-.5em}
  \centering
  \subfigure[Random weights]{\label{subfig:change_top_random}
  \includegraphics[width=.4\linewidth]{figures/change_top_N=20K=10.pdf}} 
  \subfigure[Equal weights]{\label{subfig:change_top}
  \includegraphics[width=.4\linewidth]{figures/change_top_N=20K=10random=False.pdf}} 
  %\vspace*{-.6em}
  \caption{ \textbf{Changing communication network topology.} We change the number of neighbors of each agent. (i) In Figure~\ref{subfig:change_top_random}, we randomly generalize the weights of the graph such that each row of $\mW$ sum up to 1; (ii) In Figure~\ref{subfig:change_top}, we set the non-zero entries in each row of $\mW$ all to be $\frac{1}{\text{number of neighbors}}$. We plot the curves of value functions changing with the iteration number. The green dashed line represents the optimal value. For both \ref{subfig:change_top_random} and \ref{subfig:change_top}, the convergence speed increase as number of neighbors increases. FedNPG performs better when using equal weights.
  }\label{fig:change_top}
\end{figure}

\subsection{Discussion on the Experiments}
Note that even though there are many existing works in federated RL, none of the existing works, to the best of our knowledge, studies federated multi-tasks RL in the decentralized setting. Therefore, we are not able to compare our work with existing works. However, here we include a comparison between FedNPG and a naïve baseline without the Q-tracking technique (line 6 in Algorithm~\ref{alg:DNPG_exact}).
\begin{figure}[!htb]
  \centering
  \includegraphics[width=.6\linewidth]{figures/without_tracking.pdf}
\caption{Comparison between FedNPG and a naïve baseline without the Q-tracking technique. The plot shows that while FedNPG converges within a few iterates, the algorithm without Q-tracking diverges, confirming the positive role of Q-tracking in ensuring convergence.
}\label{fig:without_tracking}
\end{figure}

For this plot, we use the standard ring graph (Eq.~\ref{eq:standard_ring}). We fix the size of the maze $K=30$, learning rate $\eta=0.1$, and regularity coefficient $\tau=0.005$. We experiment on different number of agents $N$ and plot the curves of value function changing with the iteration number. The plot shows that while FedNPG converges within a few iterates, the algorithm without Q-tracking diverges, confirming the positive role of Q-tracking in ensuring convergence.



==> related_methods.tex <==
\section{Relevant single-agent NPG methods and dynamic consensus methods in distributed learning}\label{sec_app:relevant_methods}

\textbf{Single-agent NPG methods.} Here we suppose $N=1$. Let $\eta>0$ denote the learning rate. Let $V_\tau^{(t)}$, $Q_\tau^{(t)}$ and $d_\rho^{(t)}$ denote $V_\tau^{\pi^{(t)}}$, $Q_\tau^{\pi^{(t)}}$ and $d_\rho^{\pi^{(t)}}$, resp. The NPG method with entropy regularization under tabular softmax policy parameterization in single-agent setting is summarized in Alg.~\ref{alg:npg_reg_single_exact} (see Alg.~1 in \cite{cen2022fast}).

\begin{algorithm}[H]
    \caption{Single-agent NPG with entropy regularization under softmax parameterization}
    \label{alg:npg_reg_single_exact}
    \begin{algorithmic}[1] 
        \STATE \textbf{Input:}  learning rate $\eta>0$, initialization $\pi^{(0)}$, regularization coefficient $\tau\geq 0$.
        
        \FOR{$t=0, 1, \cdots$} %%%%%%
            \STATE Compute the regularized Q-function $Q_\tau^{(t)}$ (defined in \ref{eq:Q_V}) of policy $\pi^{(t)}$.


            \STATE Update the policy:

            \begin{equation}\label{eq:update_single}
                \forall (s,a)\in \mathcal{S}\times \mathcal{A}:\quad \pi^{(t+1)}(a|s)=\frac{1}{Z^{(t)}(s)}(\pi^{(t)}(a|s))^{1-\frac{\eta\tau}{1-\gamma}}\exp{\left(\frac{\eta Q_\tau^{(t)}(s,a)}{1-\gamma}\right)}\,,
            \end{equation}
            where $Z^{(t)}(s)=\sum_{a'\in\mathcal{A}}(\pi^{(t)}(a'|s))^{1-\frac{\eta\tau}{1-\gamma}}\exp{\frac{\eta Q_\tau^{(t)}(s,a')}{1-\gamma}}$.
        \ENDFOR 
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}

We summarize the 
When the regularization coefficient $\tau=0$,  Alg.~\ref{alg:npg_reg_single_exact} is reduced to vanilla NPG, and \citet{agarwal2021theory} gives the $\mathcal{O}(1/T)$ last-iterate convergence rate and a iteration complexity of 
% $$\frac{\log |\A|}{\eta T}+\frac{1}{(1-\gamma)^2T}$$
$$\mathcal{O}\left(\frac{1}{(1-\gamma)^2\varepsilon}+\frac{1}{\eta\varepsilon}\right)$$
w.r.t. the value function for any constant learning rate $\eta>0$, when assuming exact gradient can be obtained. They also consider the case where only inexact gradient is available, and provide the $O\left(\frac{1}{(1-\gamma)\sqrt{T}}\right)$ average-iterate convergence rate when the estimation errors do not exceed certain threshold.  

When $\tau>0$, \citet{cen2022fast} proves that Alg.~\ref{alg:npg_reg_single_exact} enjoys fast linear convergence rate and has a iteration complexity of
$$\mathcal{O}\left(\frac{1}{\eta\tau}\log \left(\frac{1}{\varepsilon}\right)\right)$$
when $\eta\in (0,\frac{1-\gamma}{\tau}]$. And the best convergence guarantee is achieved when $\eta=(1-\gamma)/\tau$, where the iteration complexity reduces to 
$$\mathcal{O}\left(\frac{1}{1-\gamma}\log \left(\frac{1}{\varepsilon}\right)\right)\,.$$
They also consider the inexact version of Alg.~\ref{alg:npg_reg_single_exact} and demonstrate that their algorithm exhibits the same convergence behavior as in the exact gradient case before an approximation error floor is hit.

\textbf{Dynamic consensus methods in distributed learning.} %We invoke \textit{dynamic consensus} method, which has been effective in decentralized optimization known as gradient tracking ~\citep{qu2017harnessing,zhao2022beer,li2020communication,pu2021distributed}, to track the global average Q-function. 
To track the global average Q-function, we adopt a similar dynamic consensus scheme as the one presented in \citet{qu2017harnessing}. So to give a clearer motivation of our work, we briefly introduce the first-order distributed optimization method in \citet{qu2017harnessing} in the following. 

Same as in our case, they also consider $N$ agents who communicate through an undirected and connected communication graph that could be presented by a doubly stochastic mixing matrix $\mW=[w_{ij}]_{N\times N}$ (see Section~\ref{sec:preliminaries}). Each agent has a convex function $f_i:\RR^d\rightarrow\RR$ that is $\beta$-smooth w.r.t. $l^2$-norm. %(as per Def.~\ref{def:smoothness}). 
The objective is to find $\vx\in \RR^{1\times d}$ to minimize the average of all the functions, i.e.,
\begin{equation}\label{eq:func_sum}
    \min_{\vx\in\RR^d} f(\vx)\coloneqq\frac{1}{N}\sum_{i=1}^N f_i(\vx)\,.
\end{equation}

Each agent $i$ keeps an estimate of the minimizer $\vx_i^{(t)}\in \RR^{1\times d}$, and another vector $\vs_i^{(t)}\in \RR^{1\times d}$ which is designated to estimate the average gradient $\frac{1}{N}\sum_{i=1}^N\nabla f_i(\vx_i^{(t)})$. Define $\mX^{(t)},\mS^{(t)},\nabla^{(t)}\in\R^{N\times d}$ as
$$
\mX^{(t)}\coloneqq 
\begin{pmatrix}
    \vx_1^{(t)}\\
    \cdots\\
    \vx_N^{(t)}
\end{pmatrix}\,,\quad
\mS^{(t)}\coloneqq 
\begin{pmatrix}
    \vs_1^{(t)}\\
    \cdots\\
    \vs_N^{(t)}
\end{pmatrix}\,,\quad
\nabla^{(t)}\coloneqq 
\begin{pmatrix}
    \nabla f_1(\vx_1^{(t)})\\
    \cdots\\
    \nabla f_N(\vx_N^{(t)})
\end{pmatrix}\,.
$$
Then the algorithm in \citet{qu2017harnessing} can be summarized in Alg.~\ref{alg:distributed}.

\begin{algorithm}[H]
    \caption{Consensus-based distributed learning method in~\citet{qu2017harnessing}.}
    \label{alg:distributed}
    \begin{algorithmic}[1] 
        \STATE \textbf{Input:}  iteration number $T\in \NN_+$, learning rate $\eta>0$, mixing matrix $\mW\in\R^{N\times N}$.

        \STATE \textbf{Initialize:} $\vx_i^{(0)}\in\R^{1\times d}$, $\vs_i^{(0)}=\nabla f_i(\vx_i^{(0)})$, $i\in[N]$.
        
        \FOR{$t=0, 1, \cdots, T$} %%%%%%
            \STATE $\mX^{(t+1)}=\mW\mX^{(t)}-\eta\mS^{(t)}$

            \STATE $\mS^{(t+1)}=\mW\mS^{(t)}+\underbrace{\nabla^{(t+1)}-\nabla^{(t)}}_{\text{gradient tracking}}$
        \ENDFOR 
    \end{algorithmic}
    % \vspace*{-1em}
\end{algorithm}

\citet{qu2017harnessing} give the convergence rate of $\mathcal{O}(1/T)$ of Alg.~\ref{alg:distributed}.
